Verification of Quantitative Hyperproperties Using Trace Enumeration Relations

Many important cryptographic primitives offer probabilistic guarantees of security that can be specified as quantitative hyperproperties; these are specifications that stipulate the existence of a certain number of traces in the system satisfying certain constraints. Verification of such hyperproperties is extremely challenging because they involve simultaneous reasoning about an unbounded number of different traces. In this paper, we introduce a technique for verification of quantitative hyperproperties based on the notion of trace enumeration relations. These relations allow us to reduce the problem of trace-counting into one of model-counting of formulas in first-order logic. We also introduce a set of inference rules for machine-checked reasoning about the number of satisfying solutions to first-order formulas (aka model counting). Putting these two components together enables semi-automated verification of quantitative hyperproperties on infinite state systems. We use our methodology to prove confidentiality of access patterns in Path ORAMs of unbounded size, soundness of a simple interactive zero-knowledge proof protocol as well as other applications of quantitative hyperproperties studied in past work.

==> sections/case-studies.tex <==
\section{Microbenchmarks}
In this section we present three systems as concrete examples, which we used as our benchmarks for evaluation; present their models, define the properties that we want to prove in these systems, and discuss how we can prove these properties using the enumeration technique presented in this paper.

      %--------------------------------------------------------------------------------------------------
      %                   Balance Transfer
      %--------------------------------------------------------------------------------------------------
    \subsection{Electronic Purse}
          The amount debited is known to the adversary, as is the timing and number of successful debits.
          We prove a deniability property stating that if the amount debited is $D$, then for every trace of adversary observations, there are $D$ different initial balances which could have resulted in the same sequence of adversary observations.

    Consider the system presented in Example \ref{alg:balance-transfer}, which receives the \bal{} of a bank account as input and decrements a constant amount (\decr{}) from this account until the balance is sufficient i.e. \bal{} $\geq$ \decr{}. The program then outputs the number of decrements (\steps{}) once the execution is completed. 
    %Notice, \code{done} is \code{true} iff,  \bal{} $<$ \decr{}, and no more decrement in account balance is possible, \code{false} otherwise.

    
    \begin{algorithm}
      \DontPrintSemicolon
      \SetAlgorithmName{Example}{}{}
      \SetKwInOut{Secret}{Secret Input}
      \SetKwInOut{Output}{Public Output}
      \SetKwInOut{Constant}{Public Constant }
      
      \Secret{$balance$}
      \Output{$steps$}
      \Constant{$decr$}
      \BlankLine
    
      $steps \gets 0$ \;
      \While{balance $\geq$ decr}{
        $balance \gets balance - decr$ \;
        $steps \gets steps + 1$ \;
        {\bf print} $steps$ \;
      }

      \caption{\textsc{BalanceTransfer}}
      \label{alg:balance-transfer}
  \end{algorithm}
  
    Here, \decr{} is a publicly known constant, \bal{} is the \emph{(secret)} account balance, and \steps{} counts the number of times the amount \decr{} has been decremented from \bal{} so far. The value of the variable \steps{} is always visible to a observer. Notice that in practical use cases, the value of \steps{} need not be an output of the program, but could be a side channel vector, where an adversary observes, let's say the timing channel, to figure out the number of steps the program has executed. 

    In this program, an obvious interest lies in determining how much information about \bal{} is leaked by observing the value of \steps{}. We will define this property formally later in this section. For now, lets focus on how the execution trace of this program would look like. 
  
    \begin{figure}[h]
      \centering
      \includegraphics[width=\columnwidth]{images/balance-transfer-trace.pdf} 
      \caption{Trace of the Balance Transfer Program with initial account \code{balance = 600,000} and \code{decr = 50,000}}\label{fig:balance-transfer-trace}
    \end{figure}

    Figure \ref{fig:balance-transfer-trace} shows a trace of execution of this program on the input: \code{balance = 600,000} and \code{decr = 50,000}. The states of the program is represented by circles and the transitions from one state to another are given by arrows. Given any state $s_i$ from the trace $\pi := \langle s_0, s_1, s_2, \ldots s_n \rangle$ of a system, $obs(s_i)$ represent the values of the observable variables at the state $s_i$, in this case the value of the variable \steps{}, shown above the state and $secret(s_i)$ represent the values of the secret variables at the state $s_i$, in this case the value of  \bal{}, shown below the state.
  
    \todonote{Trim down this subsection}

    \subsubsection*{Properties to prove} 
    Observing the trace presented in Figure \ref{fig:balance-transfer-trace}, it is apparent that there is some information leak present. The number of steps the system executes can help an observer to guess a range in which the value of the variable \bal{} lies, in the starting state. As the value of \decr{} is a known constant, this allows an observer to calculate the range in which the value of \bal{} lies at each subsequent state of the given trace. The question here is, is this leak of information sufficient for an adversary to guess the exact value of \bal{}?
      
    The properties of the above form cannot be determined by observing a single trace of the system and are defined as a QHP -- which express a bound on the number of computation traces that satisfy a given relation. In this example, we want to determine, if the ``range" of the input value we get by observing a trace of the system is large enough to guess the initial value of \bal{}?  
    
    \begin{figure}[h]
      \centering
      \includegraphics[width=\columnwidth]{images/balance-transfer-traces.pdf} 
      \caption{Traces of the Balance Transfer Program demonstrating Quantitative Deniability. Here, circle represent states of a trace, and value of \steps{}  is shown above a state and value of \bal{} is shown below the state.}
      \label{fig:balance-transfer-traces}
    \end{figure}

    We can express this as a deniability property, discussed in Section \ref{sec:details} (Example \ref{ex:deniability}) -- given a computation trace of a system, $\pi := \langle s_0, s_1, s_2, \ldots s_n \rangle$, there exist at-least $k$ different traces $\pi_1, \pi_2, \ldots, \pi_k$, such that they have same value of \steps{} in corresponding states, but different values of \bal{}, as shown in Figure \ref{fig:balance-transfer-traces}. 
    

    Formally, this property can be written as:
    \begin{flalign}
      \label{eqn:deniability-balance-transfer}
      & \forall \pi.~\exists \pi_1, \dots \pi_k.~
      \Land_{j=1}^k \big( {\pi} \approx_\mathit{obs} \pi_j \land secret(\pi) \neq secret(\pi_j) \big)
    \end{flalign}
    
    \todonote{Write the property in our notation}

    \todonote{Write enumeration relation}
  %  Notationally, for a given set of observable variables (\emph{obs}), we say two states are \emph{obs-}equivalent i.e. $s_i \approx_\mathit{obs} s_j$, iff, $obs(s_i) = obs(s_j)$ and two traces $\pi_i \approx_\mathit{obs} \pi_j$, iff, $\forall m, obs(s_i^m) = obs(s_j^m)$, where $\pi_i = \langle s_i^0, s_i^1, s_i^2, \ldots s_i^n \rangle$ and $\pi_j = \langle s_j^0, s_j^1, s_j^2, \ldots s_j^n \rangle$. Then, deniability property for this program could be stated as:
  
    
  
%     In this example, the low variables are: \steps{} and \code{done} and the input is \bal{}. The computation traces shown in Figure \ref{fig:balance-transfer-traces}, capture the property of quantitative deniability, with the value low variables shown above each state and the value of high variable shown below each state, and $k = \decr{} - 2$. Notice that all the computation traces have same values for low variables and different values for high variables.
   
    
  
% \subsubsection*{Enumeration}~

%     \begin{figure}[h]
%       \centering
%       \includegraphics[width=\columnwidth]{images/balance-transfer-enumeration.pdf}
%       \caption{Given a trace (a), we can enumerate another trace (b); such that the observed values are same, although $\forall i, b_i \neq c_i$ }\label{fig:balance-transfer-enumeration}
%     \end{figure}
  
%     \begin{minipage}{0.92\linewidth}
%       \lstinputlisting[language=Python, caption=Balance Transfer Enumeration, label=code:balance-enumeration]{codes/balance-transfer-enumeration.py}
%     \end{minipage}
    
    %--------------------------------------------------------------------------------------------------
    %                   Password Checker
    %--------------------------------------------------------------------------------------------------
    \subsection{Password Checker}
    Consider the simple password checker module given in Example \ref{alg:password}. In this module, a \emph{secret} password of $n$ bits is chosen uniformly randomly, for a publicly known constant $n$. The module starts the execution with the flag $success$ set to $\false$. It then accepts password from the user and compares it with the secret password. If the user enters the correct password then the flag ($success$) is set to $\true$, else it retains its initial value  --$\false$. Notice that, usually a password checker module returns once the correct password is entered, however, here we deviate from this ideal behavior and accept $2^n$ user inputs. This ensures that the system has the execution trace of the same length, irrespective of the attempt in which the correct guess is made. The flag $success$ however, once set to $\true$ remains $\true$ throughout the execution of the module. 
    
    \begin{algorithm}
      \DontPrintSemicolon
      \SetAlgorithmName{Example}{}{}
      \SetKwInOut{Secret}{Secret Input}
      \SetKwInOut{Output}{Public Output }
      \SetKwInOut{Constant}{Public Constant }

      \Secret{$password$} 
      \tcc*[r]{chosen uniformly randomly}
      
      \BlankLine
      \Constant{$n$}
      \Output{$success$}

      \BlankLine
    
      $success \gets \false$ \;
      $attempts \gets 0$ \;
      \While{$\true$}{
        Get $inputPassword$ as user input \;
        \If{$inputPassword == password$}{
          $success \gets \true$
        }
        {\bf print} $success$ \;
      }

      \caption{\textsc{PasswordChecker}}
      \label{alg:password}
    \end{algorithm}

    Figure \ref{fig:password-trace} shows a trace of the program, where the inputs of the user are shown above the states, the value of $success$ is shown within the state, and the secret password is $p_i$, which when passed as a user input sets the boolean flag $success = \true$. The correct password $p_i$ is the secret input to the module. 

    \input{figures/password-trace.tex}

    \subsubsection*{Verification Objectives}
    In the above module, the secret password is chosen uniformly randomly for every execution of the module, hence, the probability of guessing the correct password in an attempt is $1/2^n$. Every attempt for guessing a correct password leaks some information about the password, viz. whether the password is correct or not. We would like to show however, that this information leak is not sufficient for guessing the correct password; in other words, the adversary can not do better than brute-forcing the secret password.  

    \subsubsection{Password checker security as a QHP}
    Let $M = \langle X \cup P, \minit, \mtr\land P'= P \rangle$ represent the password checking module, where $P$ is a variable that denotes the secret password and the transition relation ensures that $P$ never changes.
    Suppose $pwd(\stat{})$ denote the secret password, $obs(\stat{})$ be the term that denotes the adversary observations -- value of the flag $success$, and $inp(\stat{})$ denotes the adversary inputs in state $\stat{}$. Then the security of the password checker module can be represented by the following QHP.

    % Current approach using QNI
    % ===========================
    % This approach talks about the bit leakage for the password checker program. Here, when we allow brute forcing, then does the bit leakage makes sense?Instead, we should show that the adversary can not do better than brute force. Talking in terms of QNI makes sense, if we want to prove a bound in the bit leakage.s
    
    \begin{equation}\label{eqn:password}
      \forall \trv{0}.~\#\trv{1}: \ltlf{(\delta_{\trv{j}, \trv{k}})}.~ \ltlg{\psi_{\trv{0}, \trv{1}}} \leq 2^\mathsf{n}
    \end{equation}
    where the binary predicates $\delta$ and $\psi$ are defined as follows.
    \begin{align*}
      \delta(\stat{1}, \stat{2})  &\doteq obs(\stat{1}) \neq obs(\stat{2})\\
      \psi(\stat{1}, \stat{2})    &\doteq \left( inp(\stat{1}) = inp(\stat{2}) \right) \land \left( pwd(\stat{1}) \neq pwd(\stat{2})\right) 
    \end{align*}

    To prove the property we show that for every trace of adversary inputs for the system $M$, there are a large number of traces, upper bounded by $2^n$, having different secret password and same adversary inputs, but different adversary observations. Intuitively this implies that 

    % To prove the property we show that for every trace of $M$, there are a large number of traces ($2^n$) having the same secret password, but different adversary inputs and observations. Intuitively this implies that for a randomly chosen secret password, the adversary has $2^n$ possible different input traces, denoting the different order in which she can make her guess, with different observations. This results in the search space for the password to be exponential in the number of bits. This is depicted in Equation \ref{eqn:password}. The condition in $\delta$ denotes, that the observations and inputs of adversary is different in each of the traces captured by the counting quantifier. The requirement imposed by $\psi$ is that the secret password for all the traces captured by the counting quantifier is same as the secret password in the trace $\trv{0}$.

    \subsubsection{Verifying the password checker security}
    To verify the QHP stated in Equation \ref{eqn:password} consider a trace of the system $M$, where the secret passwords are randomly chosen from $\{0,1\}^n$, $inp[1], inp[2], \ldots inp[2^n]$ be the trace of adversary inputs, and $obs[1], obs[2], \ldots obs[2^n]$ be the trace of adversary observations. Recall that each adversary input is a guessed password, so $inp[i] \in \{0,1\}^n$ for all $i$. 
    %To generate a different trace of adversary inputs, consider an element $E \in \{0,1\}^n$, except $E = 0$. Then then the trace of inputs defined by $inp_1[i] = inp[i] \oplus E$ for $i = 1, 2, \ldots, 2^n$ will differ from the initial trace of inputs and satisfy the counting quantifier in Equation \ref{eqn:password}.
    % As different values of $E$ will result in different input traces, this defines an injective mapping from the satisfying assignemt of the following predicate to the satisfying traces of the counting quantifier. 

    % \begin{equation}
    %   \valid{E,n}{} \doteq (0 < E \leq 2^n)
    % \end{equation}
    % Hence, the number of satisfying assignments to the above formula lower bounds the number of traces satisfying the counting quantifier. In this case, counting the number of satisfying assignments to $\valid{E, n}{}$ is rather trivial, thereby bounding the number of satisfying traces for the counting quantifier by $2^n-1$.

    %--------------------------------------------------------------------------------------------------
    %                   Permutations
    %--------------------------------------------------------------------------------------------------

    \subsection{Uniform Random Permutation}
    Example \ref{alg:permutation} presents the module that takes as input an array and returns its uniform random permutation. Given a \emph{secret} array $A \doteq a_0, a_1, a_2 \ldots a_n$ the module performs an in-place permutation of $A$, by swapping all its elements ($a_i$) with another element ($a_j$) chosen randomly, such that the index of $a_i$ is greater than or equal to the index of $a_j$. For representational clarity we denote the initial array by $A$ and its permuted version by $A_p$. 

    \begin{algorithm}
      \DontPrintSemicolon
      \SetAlgorithmName{Example}{}{}
      \SetKwInOut{Secret}{Secret Input}
      \SetKwInOut{Output}{Public Output }
      
      \Secret{$A$}
      \Output{$A_p$} \tcc*[r]{Permutation of array A}

      \BlankLine
    
      n $\gets $ {\bf len}($A$)\;
      $A_p \gets A$\;
      \For{$i\leftarrow 0$ \KwTo $n$} {
        $r \gets$ {\bf random}(i, n)\;
        {\bf swap}($A_p$[$i$], $A_p$[$r$])\;
      }
        {\bf print} $A_p$ \;

      \caption{\textsc{UniformPermutation}}
      \label{alg:permutation}
    \end{algorithm}

    In the above algorithm the input array $A$ is secret and the adversary can only observe its final permuted version. The question we ask here is: can the adversary, observing the permuted array $A_p$, determine the original array $A$?

